Real-time hybrid testing using iterative control for periodic oscillations

Real-time hybrid testing is a method in which a substructure of the system is realised experimentally and the rest numerically. The two parts interact in real time to emulate the dynamics of the full system. Such experiments however are often difficult to realise as the actuators and sensors, needed to ensure compatibility and force-equilibrium conditions at the interface, can seriously affect the predicted dynamics of the system and result in stability and fidelity issues. The traditional approach of using feedback control to overcome the additional unwanted dynamics is challenging due to the presence of an outer feedback loop, passing interface displacements or forces to the numerical substructure. We, therefore, advocate for an alternative approach, removing the problematic interface dynamics with an iterative scheme to minimise interface errors, thus, capturing the response of the true assembly. The technique is examined by hybrid testing of a bench-top four-storey building with different interface configurations, where using conventional hybrid measurement techniques is very challenging. A case where the physical part exhibits nonlinear restoring force characteristics is also considered. These tests show that the iterative approach is capable of handling even scenarios which are theoretically infeasible with feedback control.

==> figs/freq_sweep_err_nl.tex <==
\begin{figure}[]
    \centering
    \begin{tabular}{cc}
        \begin{tikzpicture}
            \begin{axis}[
            xlabel={$f \; {\rm [Hz]}$},
            ylabel={$A_3 \; {\rm [m]}$},
            mark size = 1pt,
            xmin = 12.5,
            xmax = 14,
            width=0.8\textwidth,
            height=9/16*0.8\textwidth
            ]
            \addplot [blue, only marks, error bars/.cd,
            y dir=both,y explicit relative] table[x=x,y=y,y error=error] {figs/freq_sweep_nl1.dat};
            \addplot [blue, only marks, error bars/.cd,
            y dir=both,y explicit relative] table[x=x,y=y,y error=error] {figs/freq_sweep_nl2.dat};
            %\addplot [red, line width = 1pt] table {measres/sw_f_X_noise_0_up.dat};
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        &
        \begin{tabular}{c}
            \begin{tikzpicture}
                \begin{axis}[width=0.3\textwidth,ymax=30,ymin=0,xmin=0,xmax=29, xtick distance=5, minor y tick num = 1,area style]
                \addplot+[ybar interval] plot coordinates {(0, 19) (1, 14) (2, 25) (3, 10) (4, 2) (5, 3) (6, 0) (7, 1) (8, 1) (9, 1) (10, 0) (11, 2) (12, 0) (13, 1) (14, 0) (15, 2) (16, 0) (17, 1) (18, 0) (19, 1) (20, 0) (21, 0) (22, 0) (23, 0) (24, 0) (25, 0) (26, 1) (27, 1) (28, 1)};
                \end{axis}
            \end{tikzpicture}
            \\
            \begin{tikzpicture}
                \begin{axis}[
                xlabel={$F \; {\rm [N]}$},
                ylabel={$\Delta x_3 \; {\rm [m]}$},
                mark size = 1pt,
                xmin = -55,
                xmax = 55,
                width=0.3\textwidth,
                height=1.5*9/16*0.3\textwidth
                ]
                \addplot [red, line width = 1pt] table[] {figs/nl_forc_meas_n.dat};
                \addplot [red, line width = 1pt] table[] {figs/nl_forc_meas_p.dat};
                \addplot [red, line width = 1pt, densely dashed] table[] {figs/nl_forc_meas_n0.dat};
                \addplot [red, line width = 1pt, densely dashed] table[] {figs/nl_forc_meas_p0.dat};
                \addplot [blue, only marks] table[] {figs/nl_forc_meas.dat};
                %\addplot [blue, only marks, error bars/.cd,
                %y dir=both,y explicit relative] table[x=x,y=y,y error=error] {figs/freq_sweep_nl2.dat};
                %\addplot [red, line width = 1pt] table {measres/sw_f_X_noise_0_up.dat};
                %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
                %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
                \end{axis}
            \end{tikzpicture}    
        \end{tabular}
        
        
    \end{tabular}
    \caption{Comparison of frequency sweeps in case of low and high levels of measurement noise.}
    \label{tab:freq_sweep_noise}
\end{figure}

==> figs/phase_plots.tex <==
\begin{figure}[]
    \centering
    \begin{tabular}{rcl}
        \begin{tikzpicture}
            \begin{axis}[
            ylabel={$\xi_3 \; {\rm [m]}$},
            xlabel={$x_3 \; {\rm [m]}$},
            xmin = -1.6e-4,
            xmax = 1.6e-4,
            ymin = -1.6e-4,
            ymax = 1.6e-4,
            mark size = 1pt,
            width=0.3\textwidth,
            height=0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/lis_plot_BP50_p033.dat};
            \addplot [red, line width = 1.5pt] table {
                -1.6e-4 -1.6e-4
                1.6e-4 1.6e-4
            };
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        &
        \begin{tikzpicture}
            \begin{axis}[
            ylabel={$\xi_3 \; {\rm [m]}$},
            xlabel={$x_3 \; {\rm [m]}$},
            xmin = -2e-4,
            xmax = 2e-4,
            ymin = -2e-4,
            ymax = 2e-4,
            mark size = 1pt,
            width=0.3\textwidth,
            height=0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/lis_plot_BP30_nl_forw.dat};
            \addplot [red, line width = 1.5pt] table {
                -2e-4 -2e-4
                2e-4 2e-4
            };
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        &
        \begin{tikzpicture}
            \begin{axis}[
            ylabel={$\xi_3 \; {\rm [m]}$},
            xlabel={$x_3 \; {\rm [m]}$},
            xmin = -2e-4,
            xmax = 2e-4,
            ymin = -2e-4,
            ymax = 2e-4,
            mark size = 1pt,
            width=0.3\textwidth,
            height=0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/lis_plot_BP38_separate_hh.dat};
            \addplot [red, line width = 1.5pt] table {
                -2e-4 -2e-4
                2e-4 2e-4
            };
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        \\
        \begin{tikzpicture}
            \begin{axis}[
            xlabel={$t\; {\rm [s]}$},
            ylabel={$x_3, \xi_3 \; {\rm [m]}$},
            xmin=0,
            xmax=0.2,
            mark size = 1pt,
            width=0.3\textwidth,
            height=9/16*1.5*0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/time_histx_BP50_p033.dat};
            \addplot [orange, line width = 1.2pt] table {figs/time_histxi_BP50_p033.dat};
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        &
        \begin{tikzpicture}
            \begin{axis}[
            xlabel={$t\; {\rm [s]}$},
            ylabel={$x_3, \xi_3 \; {\rm [m]}$},
            xmin=0,
            xmax=0.2,
            mark size = 1pt,
            width=0.3\textwidth,
            height=9/16*1.5*0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/time_histx_BP30_nl_forw.dat};
            \addplot [orange, line width = 1.2pt] table {figs/time_histxi_BP30_nl_forw.dat};
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        &
        \begin{tikzpicture}
            \begin{axis}[
            xlabel={$t\; {\rm [s]}$},
            ylabel={$x_3, \xi_3 \; {\rm [m]}$},
            xmin=0,
            xmax=0.2,
            mark size = 1pt,
            width=0.3\textwidth,
            height=9/16*1.5*0.3\textwidth
            ]
            \addplot [blue, line width = 1pt] table {figs/time_histx_BP38_separate_hh.dat};
            \addplot [orange, line width = 1.2pt] table {figs/time_histxi_BP38_separate_hh.dat};
            %\addplot [blue, line width = 1pt] table {measres/sw_f_X_noise_0_down.dat};
            %\addplot [red, line width = 1.5pt, dashed] table {measres/amp_response_analytical_f24.dat};
            \end{axis}
        \end{tikzpicture}
        \\



    \end{tabular}
    
    %\end{tabular}
    \caption{Comparison of frequency sweeps in case of low and high levels of measurement noise.}
\end{figure}
